Approximate Capacity of Gaussian Interference-Relay Networks with Weak Cross Links

In this paper we study a Gaussian relay-interference network, in which relay (helper) nodes are to facilitate competing information flows over a wireless network. We focus on a two-stage relay-interference network where there are weak cross-links, causing the networks to behave like a chain of Z Gaussian channels. For these Gaussian ZZ and ZS networks, we establish an approximate characterization of the rate region. The outer bounds to the capacity region are established using genie-aided techniques that yield bounds sharper than the traditional cut-set outer bounds. For the inner bound of the ZZ network, we propose a new interference management scheme, termed interference neutralization, which is implemented using structured lattice codes. This technique allows for over-the-air interference removal, without the transmitters having complete access the interfering signals. For both the ZZ and ZS networks, we establish a new network decomposition technique that (approximately) achieves the capacity region. We use insights gained from an exact characterization of the corresponding linear deterministic version of the problems, in order to establish the approximate characterization for Gaussian networks.

==> DZZ-ach.tex <==
\subsection{The Achievability Proof}
\label{subsec:dzz:ach}

In this part we will show that all rate pairs satisfying inequalities
(\ref{dzz:s1})-(\ref{dzz:d1d2}) are achievable. In particular, we
introduce a coding scheme which achieves such rates. Our coding scheme
can be considered in two different phase. In the first phase, we start
with ``full $\ZZ$ pair'' in which the interference can be completely
cancelled. We continue with exploiting such links from the network,
until there remains no more full $\ZZ$ link. Then we have to deal with
different networks depends on the configuration of the original $\ZZ$
network. Not that the upper bound given by
(\ref{dzz:s1})-(\ref{dzz:d1d2}) consists two individual bounds,
\begin{align*}
R_1&\leq \min(m_{11},n_{11}),\\
R_2&\leq \min(m_{22},n_{22}),
\end{align*}
and six bounds on the sum rate. In each case we show that the two
individual rate bounds, and at least one of the sum-rate bounds are
achievable (Obviously, it can be shown that the achievable sum-rate
bound is the tight dominating one. However, we do not show
that). Before explaining the achievability scheme, we need the
following definitions.


\begin{definition}
  Consider the $\Z$ network shown in Figure~\ref{fig:dz}, with two
  transmitters $A$ and $B$, and two receivers $C$, and $D$, where $C$
  is connected to both $A$ and $B$. We call a part of a $\Z$ network a
  \emph{full $\Z$ path} if there exists a receiver node in $C$
  connected to two transmitter nodes in $A$ and $B$, and its neighbor
  in $B$, be also connected to a receiver node in $D$. One possible
  full $\Z$ path is illustrated in bold lines in Figure~\ref{fig:dz}.

\begin{figure}
\begin{center}
 	\psfrag{s1}[Bc][Bc]{$A$}
	\psfrag{s2}[Bc][Bc]{$B$}
	\psfrag{r1}[Bc][Bc]{$C$}
	\psfrag{r2}[Bc][Bc]{$D$}
\includegraphics[width=7cm]{Figs/z_full.eps}
\end{center}
\caption{A full $\Z$ path}
\label{fig:dz}
\end{figure}
\end{definition}

\begin{lemma}
  Number of full $\Z$ paths in a $\Z$ channel with direct link gains
  $n_{11}$ and $n_{22}$, and cross link gain $n_{12}$ is given by
\begin{align}
\eta_{\Z}=\min(n_{11},n_{12},n_{22},(n_{11}+n_{22}-n_{12})^+).
\end{align}
\label{lm:nu_z}
\end{lemma}

The proof of this lemma can be found in Appendix~\ref{sec:app-lm}.

\begin{definition}
A \emph{full $\ZZ$ pair} is a pair of full $\Z$ path in the two stages of a $\ZZ$ network.
\end{definition}

It is clear that the number of full $\ZZ$ pairs in a $\ZZ$ network is given by 
\begin{eqnarray}
\eta\triangleq \min(\eta_{m}, \eta_{n}), 
\end{eqnarray}
where $\eta_{m}$ and $\eta_{n}$ are the number of full $\Z$ paths in
the first and second stage of the $\ZZ$ network, respectively.

Now, we are ready to explain the achievability scheme. As stated
before, in this scheme transmission is done in two phases. We split
the messages into two parts, as
\begin{eqnarray*}
X_i=(X_i^{(N)},X_i^{(R)})
\end{eqnarray*}
where $X_i^{(N)}$ consists $\min(r_i,\eta)$ bits and the remaining
message, $X_i^{(R)}$ consists $(r_i-\eta)^+$ bits. In each of the
following phases we transmit one part of the messages.

\subsection*{First Phase of Transmission}
We partition the messages into tow In this phase, in each step we find
an arbitrary full $\ZZ$ pair and transmit one bit from $S_1$ to $D_1$,
and one bit from $S_2$ to $D_2$ using the full $\ZZ$ pair. Note that
in each full $\ZZ$ pair the interfered bit from $X_2$ at $D_1$ are the
same and can be cancelled out. Therefore, there is no interference to
deal with. Then we remove the used full $\ZZ$ pair, and continue our
procedure.  Clearly, all the channel gains are decreased by $1$, after
each step, and so $\eta_{m}$, $\eta_{n}$, and $\eta$. It can be shown
that the remaining network is still a deterministic network with shift
matrices. This can be done while $\eta>0$. In this phase we can send
any rate pair in
\begin{align}
\R{\DZZ}{N}\triangleq \{(R_1^{(N)},R_2^{(N)}): R_1^{(N)} \leq \eta, R_2^{(N)} \leq \eta\}
\end{align}
to the destinations. Therefore, the first part of the messages,
$X_1^{(N)}$ and $X_2^{(N)}$ can be transmitted in this phase.

\subsection*{Second Phase of Transmission}
As stated before, we have decreased all the channel gains by $\eta$ in
the first transmission phase. Denote by $m'_{ij}$ and $n'_{ij}$ the
channel gains of the remaining network, \emph{i.e.,}
\begin{align*}
m'_{ij}&=m_{ij}-\eta,\\
n'_{ij}&=n_{ij}-\eta.
\end{align*}
In the following, we consider all possible configuration of the
residual network, and derive an achievable rate region for the network
which we denote by $\R{\DZZ}{ach}$. In each case we show that the
outer bound coincides with the achievable rate region, and therefore
it is tight.

\begin{itemize}
\item[A. ] $\eta=m_{11}$:\\
  For such configuration, the residual network looks like the network
  shown in Figure~\ref{fig:zz_res_m11}.

\begin{figure}[hbtp]
\begin{center}
 	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$A$}
	\psfrag{r2}[Bc][Bc]{$B$}
	\psfrag{d1}[Bc][Bc]{$D_1$}
	\psfrag{d2}[Bc][Bc]{$D_2$}
%	\psfrag{a}[Bc][Bc]{$m_{22}-\eta$}
	\psfrag{b}[Bc][Bc]{$n'_{22}$}
	\psfrag{c}[Bc][Bc]{$m'_{11}$}
	\psfrag{d}[Bc][Bc]{$n'_{22}$}
%	\psfrag{e}[Bc][Bc]{$m_{21}-\eta$}
	\psfrag{f}[Bc][Bc]{$m'_{12}$}
	\psfrag{g}[Bc][Bc]{$n'_{12}$}
 	\psfrag{X_1}[Bc][Bc]{$X_1^{(R)}$}
	\psfrag{X_2}[Bc][Bc]{$X_2^{(R)}$}
%	\psfrag{Y'_1}[Bc][Bc]{$Y'_1$}
%	\psfrag{Y'_2}[Bc][Bc]{$Y'_2$}
%	\psfrag{X'_1}[Bc][Bc]{$X'_1$}
%	\psfrag{X'_2}[Bc][Bc]{$X'_2$}
%	\psfrag{Y_1}[Bc][Bc]{$Y_1$}
%	\psfrag{Y_2}[Bc][Bc]{$Y_2$}
\includegraphics[width=10cm]{Figs/zz_res_m11.eps}
\end{center}
\caption{The residual network when $\eta=m_{11}$}
\label{fig:zz_res_m11}
\end{figure}
It is clear that $S_1$ is isolated from the rest of the network, and
hence $R_1^{(R)}=0$. $S_2$ can communicate to $D_2$ as long as the two
cascaded paths support the rate. Therefore,
\begin{align}
\R{\DZZ}{R}=\{(0,R_2^{(R)}): R_2^{(R)}\leq \min(m'_{22},n'_{22})\}.
\label{zz:R:res_m11}
\end{align}

Combining this network with the full $\ZZ$ pairs, we obtain the total
achievable rate of the $\ZZ$ channel as
\begin{align}
\R{\DZZ}{ach} =\R{\DZZ}{N}+ \R{\DZZ}{R,A} = \{(R_1,R_2): 
&R_1 \leq \eta=m_{11}, \nonumber\\
&R_2\leq \eta + \min(m_{22}-\eta,n_{22}-\eta)=\min(m_{22},n_{22})\}.
\end{align}
where 
\begin{align}
\mathcal{A}+\mathcal{B}=\{a+b: a\in \mathcal{A} , b \in \mathcal{B}\},
\end{align}
for arbitrary sets $\mathcal{A}$ and $\mathcal{B}$.

This means that the any rate pair in the intersection of
(\ref{dzz:s1})-(\ref{dzz:d2}) is achievable, and the upper bound is
tight.


\item[B. ] $\eta=m_{22}$:\\
  Similar to the previous case, there is no path from $S_2$ to $D_2$
  as shown in Figure~\ref{fig:zz_res_m22}. Therefore no positive rate
  can be conveyed from $S_2$ to $D_2$. The transmission rate of the
  first pair $(S_1,D_1)$ is only bounded by the capacity of the
  cascaded links. Hence,
\begin{align}
\R{\DZZ}{R,B}=\{(R_1,0): R_1\leq \min(m'_{11},n'_{11})\}.
\label{R:zz_res_m22}
\end{align}


\begin{figure}[hbtp]
\begin{center}
 	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$R_1$}
	\psfrag{r2}[Bc][Bc]{$R_2$}
	\psfrag{d1}[Bc][Bc]{$D_1$}
	\psfrag{d2}[Bc][Bc]{$D_2$}
	\psfrag{a}[Bc][Bc]{$m'_{11}$}
	\psfrag{b}[Bc][Bc]{$n'_{11}$}
	\psfrag{d}[Bc][Bc]{$n'_{22}$}
	\psfrag{e}[Bc][Bc]{$m'_{21}$}
	\psfrag{f}[Bc][Bc]{$m'_{12}$}
	\psfrag{g}[Bc][Bc]{$n'_{12}$}
 	\psfrag{X_1}[Bc][Bc]{$X_1^{(2)}$}
	\psfrag{X_2}[Bc][Bc]{$X_2^{(2)}$}
%	\psfrag{Y'_1}[Bc][Bc]{$Y'_1$}
%	\psfrag{Y'_2}[Bc][Bc]{$Y'_2$}
%	\psfrag{X'_1}[Bc][Bc]{$X'_1$}
%	\psfrag{X'_2}[Bc][Bc]{$X'_2$}
%	\psfrag{Y_1}[Bc][Bc]{$Y_1$}
%	\psfrag{Y_2}[Bc][Bc]{$Y_2$}
\includegraphics[width=10cm]{Figs/zz_res_m22.eps}
\end{center}
\caption{The residual network when $\eta=m_{22}$}
\label{fig:zz_res_m22}
\end{figure}
Therefore the total transmission rate in this regime can be obtained by
\begin{align}
\R{\DZZ}{ach} =\R{\DZZ}{N}+ \R{\DZZ}{R,B}  = \{(R_1,R_2): 
&R_1 \leq \eta+\min(m_{11}-\eta,n_{11}-\eta)=\min(m_{11},n_{11}),\nonumber\\ 
&R_2\leq \eta= m_{22} \}.
\end{align}
It is again easy to show that $\R{\DZZ}{ach} =\R{\DZZ}{} $. Therefore,
the upper bound is tight.

\item[C. ] $\eta=n_{11}$:\\
  Similar to case B, there is no connection between $S_1$ and
  $D_1$. Therefore
\begin{align}
 \R{\DZZ}{R,C}=\{(0,R_2^{(2)}): R_2^{(2)}\leq \min(m'_{22},n'_{22})\},
\label{R:zz_res_n11}
\end{align}
and 
\begin{align}
\R{\DZZ}{ach} =\R{\DZZ}{N}+ \R{\DZZ}{R,C} = \{(R_1,R_2): 
&R_1 \leq \eta=n_{11},\nonumber\\ 
& R_2\leq \eta+\min(m_{22}-\eta,n_{22}-\eta)= \min(m_{22},n_{22})\}.
\end{align}
Hence, $\R{\DZZ}{ach} $ meets the boundary of the region characterized
by the upper bound.

\item[D. ] $\eta=n_{22}$:\\
  This case is also simple is similar to case A, since the second
  receiver is disconnected from the rest of the network. Hence,
\begin{align}
\R{\DZZ}{R,D}=\{(R_1^{(2)},0): R_1^{(2)}\leq \min(m'_{11},n'_{11})\},
\label{R:zz_res_n22}
\end{align}
and 
\begin{align}
\R{\DZZ}{ach} =\R{\DZZ}{N}+ \R{\DZZ}{R,D} = \{(R_1,R_2): 
&R_1 \leq \eta+\min(m'_{11},n'_{11})=\min(m_{11},n_{11}), \nonumber\\
&R_2\leq\eta= n_{22}\}.
\end{align}
This means that $\R{\DZZ}{} $ includes $\R{\DZZ}{ach}$, and the upper
bound is tight.

\item[E. ] $\eta=m_{12}$:\\
  The residual network in this regime is a pair of parallel
  independent point-to-point channels followed by a Z-channel.  Such
  network is shown in Figure~\ref{fig:zz_res_m12}.


\begin{figure}[hbtp]
\begin{center}
 	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$R_1$}
	\psfrag{r2}[Bc][Bc]{$R_2$}
	\psfrag{d1}[Bc][Bc]{$D_1$}
	\psfrag{d2}[Bc][Bc]{$D_2$}
	\psfrag{a}[Bc][Bc]{$m'_{11}$}
	\psfrag{b}[Bc][Bc]{$n'_{11}$}
	\psfrag{c}[Bc][Bc]{$m'_{22}$}
	\psfrag{d}[Bc][Bc]{$n'_{22}$}
%	\psfrag{e}[Bc][Bc]{$m_{21}-\eta$}
	\psfrag{g}[Bc][Bc]{$n'_{12}$}
 	\psfrag{X_1}[Bc][Bc]{$X_1^{(2)}$}
	\psfrag{X_2}[Bc][Bc]{$X_2^{(2)}$}
%	\psfrag{Y'_1}[Bc][Bc]{$Y'_1$}
%	\psfrag{Y'_2}[Bc][Bc]{$Y'_2$}
%	\psfrag{X'_1}[Bc][Bc]{$X'_1$}
%	\psfrag{X'_2}[Bc][Bc]{$X'_2$}
%	\psfrag{Y_1}[Bc][Bc]{$Y_1$}
%	\psfrag{Y_2}[Bc][Bc]{$Y_2$}
\includegraphics[width=10cm]{Figs/zz_res_m12.eps}
\end{center}
\caption{The residual network when $\eta=m_{12}$}
\label{fig:zz_res_m12}
\end{figure}

The achievable rate region of this network is obtained as the
intersection of the rate region of the parallel channels and the
$\Z$-channel.

\begin{align}
\R{\DZZ}{R,E}=&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq m'_{11}, R_2^{(2)} \leq m'_{22}\} \nonumber\\
&\bigcap\nonumber\\
&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq n'_{11}, R_2^{(2)} \leq n'_{22}, R_1^{(2)}+R_2^{(2)} \leq \max(n'_{11}, n'_{12})+(n'_{22}-n'_{12})^+ \}
\label{zz:R:res3}
\end{align}
We can obtain the total rate of the $\ZZ$ network by adding up the two
achievable rate pairs.

\begin{align}
  \R{\DZZ}{ach} =&\R{\DZZ}{N}+ \R{\DZZ}{R,E}\nonumber\\
  = &\{(R_1,R_2):  R_1 \leq m'_{11}+\eta, R_2\leq m'_{22}+\eta\}\nonumber\\
  &\bigcap\nonumber\\
  &\{(R_1,R_2): R_1 \leq n'_{11}+\eta, R_2 \leq n'_{22}+\eta, R_1+R_2 \leq \max(n'_{11}, n'_{12})+(n'_{22}-n'_{12})^++2\eta \}\nonumber\\
  =&\{(R_1,R_2): R_1 \leq \min(m_{11},n_{11}), \nonumber\\
  & \phantom{\{(R_1,R_2):}R_2 \leq \min(m_{22},n_{22}), \nonumber\\
  & \phantom{\{(R_1,R_2):} R_1+R_2 \leq \max(n_{11},
  n_{12})+(n_{22}-n_{12})^++m_{12} \}.
\end{align}
Note that in the last equality we have replaced $\eta$ by $m_{12}$,
and used the facts that $\max(a-c,b-c)=\max(a,b)-c$, and
$(a-b)=((a-c)-(b-c))$.
%Therefore, the individual rate inequalities are similar to (\ref{zz:s1})-(\ref{zz:d2}). The sum rate inequality can be written as
%\begin{align}
% R_1+R_2 \leq \min (m_{11},\eta)+ \min(n_{22},\eta)+ \max((m_{11}-\eta)^+, m_{12}-\eta)+ (m_{22}- m_{12})^+.
%\label{eq:zz:tot3}
%\end{align}
%In order to prove (\ref{eq:zz:tot3}) meets either (\ref{zz:s1s2}) or (\ref{zz:d1d2}), we consider the following cases.
%
%\begin{description}
% \item [$C$-I:] $ m_{11} \geq \eta, n_{22} \geq \eta$\\
%In this regime, the sum rate upper bound (\ref{eq:zz:tot3}) converts to 
%\begin{align}
% R_1+R_2 &\leq \eta+ \eta+ \max(m_{11}-\eta, m_{12}-\eta)+ (m_{22}- m_{12})^+\nonumber\\
%&= \eta + \max(m_{11}, m_{12}) +(m_{22}- m_{12})^+
%\label{eq:zz:tot3_1}
%\end{align}
%which is exactly the bound given by (\ref{zz:s1s2}). Thus the obtained strategy meets the upper bound.
%
%\item [$C$-II:] $ m_{11} \geq \eta, n_{22} \leq \eta$\\
%Rewriting the RHS of (\ref{eq:zz:tot3}) using the current assumption, we have
%\begin{align}
%\eta &+ n_{22}+ \max(m_{11}-\eta, m_{12}-\eta)+ (m_{22}- m_{12})^+\nonumber\\
%&= n_{22} + \max(m_{11}, m_{12}) +(m_{22}- m_{12})^+\nonumber\\
%&\geq n_{22} + m_{11}.
%\label{eq:zz:tot3_2}
%\end{align}
%which is not stronger than the sum-rate bound obtained by (\ref{zz:s1}) and (\ref{zz:d2}).
%That means in this regime, the achievable region includes the region specified by inequalities (\ref{zz:s1})-(\ref{zz:d2}), and the proposed strategy achieves the desired performance.
%
%\item [$C$-III:] $ m_{11} \leq \eta, n_{22} \geq \eta$\\
%We can write the RHS of (\ref{eq:zz:tot3}) as
%\begin{align}
%m_{11} &+ \eta +  (m_{12}-\eta) + (m_{22}- m_{12})^+\nonumber\\
%&= m_{11} + \max(m_{12}, m_{22}) \nonumber\\
%&\geq m_{11} + m_{22}.
%\label{eq:zz:tot3_3}
%\end{align}
%This means that this bound is not stronger than the bound obtained by (\ref{zz:s1}) and (\ref{zz:s2}).
Therefore this region includes the region specified by
(\ref{dzz:s1})-(\ref{dzz:d2}), and our strategy is optimal to meet the
upper bound.

%\item [$C$-IV:] $ m_{11} \leq \eta, n_{22} \leq \eta$\\
%Rewriting the RHS of (\ref{eq:zz:tot3}) based on our assumption in this regime, we get
%\begin{align}
%m_{11}+ n_{22} + ( m_{12}-\eta)+ (m_{22}- m_{12})^+ \geq m_{11}+n_{22}.
%\label{eq:zz:tot3_4}
%\end{align}
%which is not stronger than combination of (\ref{zz:s1}) and (\ref{zz:d2}).
%Therefore the proposed strategy can achieve any rate which satisfies (\ref{zz:s1})-(\ref{zz:d2}), and therefore is optimal.
%\end{description}


\item[F. ] $\eta=n_{12}$:\\
  In this regime we have to determine the capacity of the network
  shown in Figure~\ref{fig:zz_res_n12}, which a cascade system of a
  $\Z$-channel and a set of parallel channels. Similar to the last
  case, the rate region of this network can be written as
\begin{align}
\R{\DZZ}{R,F}
=&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq m'_{11},  R_2^{(2)} \leq m'_{22},%\nonumber\\
%& \hspace{50pt} 
R_1^{(2)}+R_2^{(2)} \leq \max(m'_{11},m'_{12})+ (m'_{22}-m'_{12})^+ \}\nonumber\\
&\bigcap\nonumber\\
&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq n'_{11},  R_2^{(2)} \leq n'_{22}\}.
%\label{zz:R:res4}
\end{align}
The total achievable rates by combining the full zz pairs and the
residual network can be characterized as follows.
\begin{align}
\R{\DZZ}{ach} =&\R{\DZZ}{N}+ \R{\DZZ}{R,F}   \nonumber\\
=&\{(R_1,R_2): R_1 \leq m'_{11}+\eta,  R_2 \leq m'_{22}+\eta, %\nonumber\\
%& \hspace{50pt} 
R_1+R_2 \leq \max(m'_{11},m'_{12})+ (m'_{22}-m'_{12})^+ +2\eta\}\nonumber\\
&\bigcap\nonumber\\
&\{(R_1,R_2): R_1 \leq n'_{11}+\eta,  R_2 \leq n'_{22}+\eta\}\nonumber\\
=&\{(R_1,R_2): R_1 \leq \min(m_{11},n_{11}),  \nonumber\\
&\phantom{\{(R_1,R_2): } R_2 \leq \min(m_{22},n_{22}), \nonumber\\
%& \hspace{50pt} 
&\phantom{\{(R_1,R_2): } R_1+R_2 \leq \max(m_{11},m_{12})+ (m_{22}-m_{12})^+ +n_{12}\}
%\label{zz:R:res4}
\end{align}

\begin{figure}[hbtp]
\begin{center}
 	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$R_1$}
	\psfrag{r2}[Bc][Bc]{$R_2$}
	\psfrag{d1}[Bc][Bc]{$D_1$}
	\psfrag{d2}[Bc][Bc]{$D_2$}
	\psfrag{a}[Bc][Bc]{$m'_{11}$}
	\psfrag{b}[Bc][Bc]{$n'_{11}$}
	\psfrag{c}[Bc][Bc]{$m'_{22}$}
	\psfrag{d}[Bc][Bc]{$n'_{22}$}
	\psfrag{f}[Bc][Bc]{$m'_{12}$}
%	\psfrag{g}[Bc][Bc]{$n'_{12}$}
 	\psfrag{X_1}[Bc][Bc]{$X_1^{(2)}$}
	\psfrag{X_2}[Bc][Bc]{$X_2^{(2)}$}
%	\psfrag{Y'_1}[Bc][Bc]{$Y'_1$}
%	\psfrag{Y'_2}[Bc][Bc]{$Y'_2$}
%	\psfrag{X'_1}[Bc][Bc]{$X'_1$}
%	\psfrag{X'_2}[Bc][Bc]{$X'_2$}
%	\psfrag{Y_1}[Bc][Bc]{$Y_1$}
%	\psfrag{Y_2}[Bc][Bc]{$Y_2$}
\includegraphics[width=10cm]{Figs/zz_res_n12.eps}
\end{center}
\caption{The residual network when $\eta=n_{12}$}
\label{fig:zz_res_n12}
\end{figure}
Since $\Rc^U\subseteq\Rc^I$, our upper bound is tight.
%
%We can determine the achievable rate pair of the original network by adding the rates of the diamond and residual networks.
%\begin{align}
%\R^{I} =\Rc_{D} + \Rc_{R,D}& \nonumber\\
%= \{(R_1,R_2): & R_1 \leq \min (m_{11},\eta)+\min((m_{11}-\eta)^+,n_{11}-\eta)\nonumber\\
%& R_2\leq \min(n_{22},\eta)+ \min(m_{22}-\eta, (n_{22}-\eta)^+ ),\nonumber\\
%& R_1+R_2 \leq \min (m_{11},\eta)+ \min(n_{22},\eta)+ \max(n_{11}-\eta, n_{12}-\eta)+ (n_{22}-\eta)^+\nonumber\\
%&\phantom{R_1+R_2 \leq } -\min((n_{22}-\eta)^+, n_{12}-\eta)\}.
%\end{align}
%It is easy to show that 
%\begin{align*}
%\min (m_{11},\eta)+\min((m_{11}-\eta)^+,n_{11}-\eta)&=\min(m_{11},n_{11})\\
%\min(n_{22},\eta)+ \min(m_{22}-\eta, (n_{22}-\eta)^+ )&= \min(m_{22},n_{22}).
%\end{align*}
%and therefore the proposed strategy can achieve the maximum individual rates. In the following we consider four different cases, and show that the sum-rate bound here
%\begin{align}
%R_1+R_2 \leq \min (m_{11},\eta)+ \min(n_{22},\eta)+ \max(n_{11}, n_{12}) -\eta + (n_{22}-\eta)^+ -\min((n_{22}-\eta)^+, n_{12}-\eta)
%\label{eq:zz:tot4}
%\end{align}
%meets one of the sum-rate bound in the upper bound given by (\ref{zz:s1})-(\ref{zz:d1d2}). 
%
%%\end{itemize}
%\begin{description}
% \item[$D$-I:]  $ m_{11}\geq \eta, n_{22} \geq \eta$:\\
%Using this assumption, we can write the RHS of sum-rate (\ref{eq:zz:tot4}) as
%\begin{align}
%\eta&+\eta + \max(n_{11}, n_{12}) -\eta + (n_{22}-\eta) -\min(n_{22}-\eta, n_{12}-\eta)\nonumber\\
%&=  \max(n_{11}, n_{12}) + n_{22} -\min(n_{22}, n_{12})+\eta\nonumber\\
%&=\max(n_{11}, n_{12}) + (n_{22}-n_{12})^+ + m_{12}
%\label{eq:zz:tot4_1}
%\end{align}
%which is exactly the same as RHS of (\ref{zz:d1d2}). Therefore the achievable region includes the outer bound, and both bounds are tight.
%
%\item [$D$-II:] $ m_{11} \geq \eta, n_{22} \leq \eta$:\\
%Rewriting the RHS of (\ref{eq:zz:tot4}) using the current assumptions, we have
%\begin{align}
%\eta + n_{22}+ \max(n_{11}, n_{12}) -\eta \geq n_{22} + n_{11}
%\label{eq:zz:tot4_2}
%\end{align}
%That means we can achieve the sum rate obtained by (\ref{zz:d1}) and (\ref{zz:d2}), and therefore the bound are tight.
%
%\item [$D$-III:] $ m_{11} \leq \eta, n_{22} \geq \eta$:\\
%We can write the RHS of (\ref{eq:zz:tot4}) as
%\begin{align}
%m_{11} &+ \eta +  \max(n_{11}, n_{12}) -\eta + (n_{22}-\eta) -\min(n_{22}-\eta, n_{12}-\eta)\nonumber\\
%&= m_{11} + \max(n_{11}, n_{12}) + n_{22}-\min(n_{22},n_{12}) \nonumber\\
%&\geq m_{11} + n_{22}.
%\label{eq:zz:tot4_3}
%\end{align}
%Note that the last inequality holds since $\max(a,b)-\min(b,c)\geq 0$ for all $a,b,c\in\mathbb{R}$. (\ref{eq:zz:tot4_3}) shows that the proposed scheme can achieve the sum rate up to the bound obtained by (\ref{zz:s1}) and (\ref{zz:d2}). Therefore all the rate pairs satisfying the upper bound are achievable. 
%
%\item [$D$-IV:] $ m_{11} \leq \eta, n_{22} \leq \eta$:\\
%Rewriting the RHS of (\ref{eq:zz:tot4}) based on our assumption in this regime, we get
%\begin{align}
%m_{11}+ n_{22} + \max(n_{11}, n_{12}) -\eta \geq m_{11}+n_{22}
%\label{eq:zz:tot4_4}
%\end{align}
%which is a consequence of the bounds (\ref{zz:s1}) and (\ref{zz:d2}). It is clear that our scheme can achieve all rate pairs satisfying the upper bound, and therefore the inner and outer bounds coincide.
%
%\end{description}

\item[G. ] $\eta=(m_{11}+m_{22}-m_{12})^+$:\\
  This following cases might be most interesting cases in
  achievability of the $\ZZ$ network. Here, we assume that after
  $\eta$ iteration of the first phase of the transmission and
  decreasing the channel gains by $\eta$ (or from the beginning of the
  transmission), we have $m'_{11}+m'_{22}-m'_{12}\leq 0$. This
  inequality means that the two messages received by $R_1$ (from $D_1$
  and $D_2$) do not interfer, and can be decoded
  separately. Figure\ref{fig:zz_res_G1} shows this phenomenon.

  As it is clear from Figure~\ref{fig:zz_res_G1}, both messages
  $X_1^{(2)}$, and $X_2^{(2)}$ can be decoded by $R_1$ and $X_2^{(2)}$
  can be decoded by $R_2$ if and only if $R_1^{(2)}\leq m'_{11}$ and
  $R_2^{(2)}\leq m'_{22}$.

\begin{figure}[ht]
\begin{center}
\subfigure[Transmission from Sources to Relays]{\label{fig:zz_res_G1}
	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$R_1$}
	\psfrag{r2}[Bc][Bc]{$R_2$}
    \psfrag{n11}[Bc][Bc]{$m_{11}$}
	\psfrag{n12}[Bc][Bc]{$m_{12}$}
	\psfrag{n22}[Bc][Bc]{$m_{22}$}
	\includegraphics[height=9cm]{Figs/zz_res_G1.eps}}
%\hspace{5mm} 
\subfigure[Transmission from Relays to Destinations]{\label{fig:zz_res_G2}
	\psfrag{s1}[Bc][Bc]{$R_1$}
	\psfrag{s2}[Bc][Bc]{$R_2$}
	\psfrag{r1}[Bc][Bc]{$D_1$}
	\psfrag{r2}[Bc][Bc]{$D_2$}
    \psfrag{n11}[Bc][Bc]{$n_{11}$}
	\psfrag{n12}[Bc][Bc]{$n_{12}$}
	\psfrag{n22}[Bc][Bc]{$n_{22}$}
	\includegraphics[height=9cm]{Figs/zz_res_G2.eps}}
\caption{Encoding scheme for the second phase of communication in regime G, when $\eta=(m_{11}+m_{22}-m_{12})^+$. interference 
Neutralization helps $D_1$ to decode its message.} 
\label{fig:zz_res_G}
\end{center}
\end{figure}


Now, in the second stage of the transmission (from relays to
destinations),we convey up to $n'_{22}$ bits from $R_2$ to $D_2$. This
transmission may make some of the levels of $D_1$ attacked by the bits
of $X_2^{(2)}$ sent by $R_2$ (as interference). $R_1$ can cancel out
this interference by adding the corresponding bits of $X_2^{(2)}$ to
its transmitted bits about $X_1^{(2)}$, as shown in
Figure~\ref{fig:zz_res_G2}. The non-interfered levels of $D_1$ can be
simply used by $R_1$ to transmit bits of $X_1^{(2)}$. Therefore, we
can send up to $n'_{11}$ bits to $D_1$ and $n'_{22}$ bits to
$D_2$. Note that important fact here is that the second message can be
completely decoded by $R_1$.

Since the encoding scheme in the two stages of communication are
independent, the achievable rate pairs of the residualnetwork can be
written as an intersection as
\begin{align}
 \R{\DZZ}{R,G} =&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq m'_{11},  R_2^{(2)} \leq m'_{22}\}\nonumber\\
&\bigcap\nonumber\\
&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq n'_{11},  R_2^{(2)} \leq n'_{22}\}\nonumber\\
=&\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq \min(m'_{11},n'_{11}), R_2^{(2)} \leq  \min(m'_{22},n'_{22})\}.
% \label{zz:R:res4}
\end{align}
Therefore the total achievable of the $\ZZ$ network would be 
\begin{align}
\R{\DZZ}{ach} &=\R{\DZZ}{N}+ \R{\DZZ}{R,G}\nonumber\\
&=\{(R_1,R_2): R_1 \leq \min(m'_{11},n'_{11})+\eta, R_2\leq  \min(m'_{22},n'_{22})+\eta\}\nonumber\\
&=\{(R_1,R_2): R_1 \leq \min(m_{11},n_{11}), R_2\leq  \min(m_{22},n_{22})\},
%\label{zz:R:res4}
\end{align}
which includes the region characterized by
(\ref{dzz:s1})-(\ref{dzz:d2}). This shows that the upper bound is
tight.

\item[H. ] $\eta=(n_{11}+n_{22}-n_{12})^+$:\\
  We can think of this case as the dual of case G. Here, the two
  messages sent by $R_1$ and $R_2$ are received by $D_1$ at different
  levels. This means the first decoder can decode the message of the
  second source, $X_2^{(2)}$ completely. Therefore it can subtract this
  message from the signal received from $R_1$, and remove the
  interference, if there is any.

  This leads to a simple communication scheme as follows. $S_1$ and
  $S_2$ broadcast their source bits to the relays arbitrarily, up to
  rates $R_1^{(2)}\leq \min(m'_{11},n'_{11})$ and $R_2^{(2)}\leq
  \min(m'_{22},n'_{22})$. Then $R_1$ and $R_2$ amplify and forward
  their received messages to $D_1$ and $D_2$. While the second message
  will be delivered to both decoders without interference, only an
  interfered version of the first message (a function of $X_1^{(2)}$
  and $X_2^{(2)}$) will be received at $D_1$. However, since the MAC
  operation is assumed to be invertible, $D_1$ can decode $X_1^{(2)}$
  having the received function and $X_2^{(2)}$.
  Figure~\ref{fig:zz_res_H} illustrates the transmission model for
  this regime. Therefore, the achievable rate pairs of the residual
  network would be
\begin{align}
\R{\DZZ}{R,H} 
=\{(R_1^{(2)},R_2^{(2)}): R_1^{(2)} \leq \min(m'_{11},n'_{11}), R_2^{(2)} \leq  \min(m'_{22},n'_{22})\}.
%\label{zz:R:res4}
\end{align}
The total rate pair achieved by the $\ZZ$ network is obtained as
\begin{align}
\R{\DZZ}{ach} &=\R{\DZZ}{N}+ \R{\DZZ}{R,H} \nonumber\\
&=\{(R_1,R_2): R_1 \leq \min(m'_{11},n'_{11})+\eta, R_2\leq  \min(m'_{22},n'_{22})+\eta\}\nonumber\\
&=\{(R_1,R_2): R_1 \leq \min(m_{11},n_{11}), R_2\leq  \min(m_{22},n_{22})\},
%\label{zz:R:res4}
\end{align}
and $\R{\DZZ}{ach} =\R{\DZZ}{}$, and the upper bound is tight.  
\begin{figure}[ht!]
\begin{center}
\subfigure[Transmission from Sources to Relays]{\label{fig:zz_res_H1}
	\psfrag{s1}[Bc][Bc]{$S_1$}
	\psfrag{s2}[Bc][Bc]{$S_2$}
	\psfrag{r1}[Bc][Bc]{$R_1$}
	\psfrag{r2}[Bc][Bc]{$R_2$}
    \psfrag{n11}[Bc][Bc]{$m_{11}$}
	\psfrag{n12}[Bc][Bc]{$m_{12}$}
	\psfrag{n22}[Bc][Bc]{$m_{22}$}
	\includegraphics[height=9cm]{Figs/zz_res_H1.eps}}
%\hspace{5mm} 
\subfigure[Transmission from Relays to Destinations]{\label{fig:zz_res_H2}
	\psfrag{s1}[Bc][Bc]{$R_1$}
	\psfrag{s2}[Bc][Bc]{$R_2$}
	\psfrag{r1}[Bc][Bc]{$D_1$}
	\psfrag{r2}[Bc][Bc]{$D_2$}
    \psfrag{n11}[Bc][Bc]{$n_{11}$}
	\psfrag{n12}[Bc][Bc]{$n_{12}$}
	\psfrag{n22}[Bc][Bc]{$n_{22}$}
	\includegraphics[height=9cm]{Figs/zz_res_H2.eps}}
\caption{Encoding scheme for the second phase of communication in regime H, when $\eta=(n_{11}+n_{22}-n_{12})^+$. $D_1$ 
decodes the common message and remove it.} 
\label{fig:zz_res_H}
\end{center}
\end{figure}


\end{itemize}

\noindent\emph{Remark. } In general the sum-rate inequalities might be
loose, or a consequence of the individual rate bounds.  It can be
shown that (\ref{dzz:s1s2}) is the dominating one only in the regime
F, \emph{i.e.,} when $\eta=n_{12}$. Similarly, the bound given in
(\ref{dzz:d1d2}) influences the rate region only when $\eta=m_{12}$
(regime E).

